Leveraging Sparse and Dense Feature Combinations for Sentiment Classification

Neural networks are one of the most popular approaches for many natural language processing tasks such as sentiment analysis. They often outperform traditional machine learning models and achieve the state-of-art results on most tasks. However, many existing deep learning models are complex, difficult to train and provide a limited improvement over simpler methods. We propose a simple, robust and powerful model for sentiment classification. This model outperforms many deep learning models and achieves comparable results to other deep learning models with complex architectures on sentiment analysis datasets. We publish the code online.

==> neural_fig.tex <==
% \begin{figure*}[!th]
%     \centering
    
%     \includegraphics[width=0.9\textwidth]{senti_lstm}
%     \caption{\footnotesize A graphical depiction of the neural network model in our direct transfer approach. This is an example of an English tweet translated to German. The words are shown at the bottom with their translation appearing after colon (``:''). The first and the last words are emojies. The circles ($f_i$) show the embedding layer, the LSTMs are shown on top of the embedding layer and the average pool layer on the right side of the words. All the intermediate layers are concatenated and fed to a multi-layer perceptron  (MLP). More details are given in \S\protect\ref{sec_direct}.}
%     \label{fig_neural_fig}
% \end{figure*}

\begin{SCfigure*}
\includegraphics[width=0.70\textwidth]{senti_lstm}
\caption{\footnotesize A graphical depiction of the neural network model in our direct transfer approach. This is an example of an English tweet translated to German. The words are shown at the bottom with their translation appearing after colon (``:'') for which underlined words are not translated. The circles ($f_i$) show the embedding layer, the LSTMs are shown on top of the embedding layer and the average pool layer on the right side of the words. All the intermediate layers are concatenated and fed to a multi-layer perceptron  (MLP). More details are given in \S\protect\ref{sec_direct}.}\label{fig_neural_fig}
\end{SCfigure*}

==> pos.tex <==
\begin{table}
\begin{tabular}{|l|l|}
\hline
& Parts of Speech \\
\hline
Nouns & NNS, NN, NNP, NNPS\\
\hline
Verbs/Prepositions & \begin{tabular}[l]{@{}c@{}}VBP, VBZ, VBG, VBD, \\VB, VBN, MD, IN\end{tabular} \\
\hline
Adverbs/Adjectives & \begin{tabular}[l]{@{}c@{}}RB, RBR, RBS, \\JJR, JJ, JJS\end{tabular}\\
\hline
\end{tabular}
\caption{Part of Speech Groups for Documents}
\label{table:doc_groups}
\end{table}

==> pos_twt.tex <==
\begin{table}
\begin{tabular}{|l|l|}
\hline
& Parts of Speech \\
\hline
Nouns & \begin{tabular}[l]{@{}c@{}}N, O, \textnormal{\^}, Z, S, M, P, X, \\\#, @, \textnormal{\~}, U, G\end{tabular}\\
\hline
Verbs/Prepositions & V, T, L\\
\hline
Adverbs/Adjectives & A, !, R, E\\
\hline
\end{tabular}
\caption{Part of Speech Groups for Twitter}
\label{table:twitter_groups}
\end{table}
